ShapeICP: Iterative Category-level Object Pose and Shape Estimation from Depth

Category-level object pose and shape estimation from a single depth image has recently drawn research attention due to its potential utility for tasks such as robotics manipulation. The task is particularly challenging because the three unknowns, object pose, object shape, and model-to-measurement correspondences, are compounded together, but only a single view of depth measurements is provided. Most of the prior work heavily relies on data-driven approaches to obtain solutions to at least one of the unknowns, and typically two, risking generalization failures if not designed and trained carefully. The shape representations used in the prior work also mainly focus on point clouds and signed distance fields (SDFs). In stark contrast to the prior work, we approach the problem using an iterative estimation method that does not require learning from pose-annotated data. Moreover, we construct and adopt a novel mesh-based object active shape model (ASM), which additionally maintains vertex connectivity compared to the commonly used point-based object ASM. Our algorithm, ShapeICP, is based on the iterative closest point (ICP) algorithm but is equipped with additional features for the category-level pose and shape estimation task. Although not using pose-annotated data, ShapeICP surpasses many data-driven approaches that rely on pose data for training, opening up a new solution space for researchers to consider.

==> includes/defense.tex <==
\begin{table*}
\begin{center}
\caption{Benchmarking results on NOCS REAL \cite{wang2019normalized}. Baseline results are from sources \cite{irshad2022shapo, akizuki2021asm}. S.D. stands for shape-annotated data required for training and P.D. stands for pose-annotated data required for training. S.C. stands for the shape classification network. The results are roughly in the order of overall performance. The best result in each metric is in bold.}
\label{tab: nocsposebrief}
    \begin{tabular}{|l| c c | c c c c|}
        \hline
        Method & \makecell{Pose\\Data} & \makecell{Shape\\Data} & \makecell{IoU25\\(\%)} & \makecell{IoU75\\(\%)} & \makecell{5\degree 5cm\\(\%)} & \makecell{10\degree 5cm\\(\%)} \\
        \hline
        \hline
        NOCS & \checkmark & \checkmark & \bf{84.8} & 30.1 & 10.0 & 25.2 \\
        \hline
        Synthesis & \hfill & \hfill & -- & -- & 0.9 & 2.4 \\
        \hline
        Metric Scale & \checkmark & \checkmark & 81.6 & -- & 5.3 & 24.7 \\
        \hline
        ASM-Net w/o ICP & \checkmark & \checkmark & -- & 31.7 & 12.4 & 37.7 \\
        \hline
        \bf{ShapeICP (Ours) w/o S.C.} & \hfill & \hfill & 81.7 & 32.9 & 25.7 & 37.9 \\
        \hline
        ASM-Net w/ ICP & \checkmark & \checkmark & -- & 37.4 & 25.6 & 43.7 \\
        \hline
        \bf{ShapeICP (Ours) w/ S.C.} & \hfill & \checkmark & 81.6 & 38.2 & \bf{31.7} & 47.1 \\
        \hline
        ShapePrior & \checkmark & \checkmark & 81.2 & \bf{53.2} & 21.4 & 54.1 \\
        \hline
        CenterSnap & \checkmark & \checkmark & 83.5 & -- & 27.2 & \bf{58.8} \\
        \hline
    \end{tabular}
\end{center}
\end{table*}

\begin{table*}
\begin{center}
\caption{Shape estimation results on NOCS REAL \cite{wang2019normalized} evaluated with Chamfer distance ($10^{-3}$). Baseline results are from sources \cite{irshad2022shapo, akizuki2021asm}. S.D. stands for shape-annotated data required for training and P.D. stands for pose-annotated data required for training. S.C. stands for the shape classification network. The results are roughly in the order of overall performance.}
\label{tab: nocsshapefull}
    \begin{tabular}{|l| c c | c c c c c c c|}
        \hline
        Method & \makecell{Pose\\Data} & \makecell{Shape\\Data} & Bottle & Bowl & Camera & Can & Laptop & Mug & Mean \\
        \hline
        \hline
        ShapePrior & \checkmark & \checkmark & 5.0 & 1.2 & 9.9 & 2.4 & 7.1 & 0.97 & 4.4 \\
        \hline
        \bf{ShapeICP (Ours) w/o S.C.} & \hfill & \hfill & 3.5 & 1.0 & 9.0 & 3.0 & 3.9 & 3.1 & 3.9 \\
        \hline
        Reconstruction & \checkmark & \checkmark & 3.4 & 1.2 & 8.9 & 1.5 & 2.9 & 1.0 & 3.2 \\
        \hline
        \bf{ShapeICP (Ours) w/ S.C.} & \hfill & \checkmark & 4.1 & 0.96 & 7.2 & 1.4 & 1.2 & 3.2 & 2.9 \\      
        \hline
        CenterSnap & \checkmark & \checkmark & 1.3 & 1.0 & 4.3 & 0.9 & 0.7 & 0.6 & 1.5 \\
        \hline
        ASM-Net & \checkmark & \checkmark & 0.23 & 0.06 & 0.61 & 0.15 & 0.60 & 0.10 & 0.29 \\
        \hline
    \end{tabular}
\end{center}
\end{table*}

\begin{table*}
\begin{center}
\caption{Shape estimation results on NOCS REAL \cite{wang2019normalized} evaluated with Chamfer distance ($10^{-3}$). Baseline results are from sources \cite{irshad2022shapo, akizuki2021asm}. S.D. stands for shape-annotated data required for training and P.D. stands for pose-annotated data required for training. S.C. stands for the shape classification network. The results are roughly in the order of overall performance.}
\label{tab: nocsshapebrief}
    \begin{tabular}{|l| c c | c |}
        \hline
        Method & \makecell{Pose\\Data} & \makecell{Shape\\Data} & \makecell{Mean\\($10^{-3}$)} \\
        \hline
        \hline
        ShapePrior & \checkmark & \checkmark & 4.4 \\
        \hline
        \bf{ShapeICP (Ours) w/o S.C.} & \hfill & \hfill & 3.9 \\
        \hline
        Reconstruction & \checkmark & \checkmark & 3.2 \\
        \hline
        \bf{ShapeICP (Ours) w/ S.C.} & \hfill & \checkmark & 2.9 \\      
        \hline
        CenterSnap & \checkmark & \checkmark & 1.5 \\
        \hline
        ASM-Net & \checkmark & \checkmark & 0.29 \\
        \hline
    \end{tabular}
\end{center}
\end{table*}

\begin{table*}
\begin{center}
\caption{Ablation results on NOCS REAL \cite{wang2019normalized}. Shape is evaluated with Chamfer distance ($10^{-3}$)}
\label{tab: ablationdefense}
    \begin{tabular}{|l| c c c c|}
        \hline
        Variation & IoU50 $\uparrow$ & 5\degree 5cm $\uparrow$ & 10\degree 5cm $\uparrow$ & shape $\downarrow$ \\
        \hline
        \hline
        No EM & -2.0 & -5.0 & -0.6 & +0.05 \\
        \hline
        No Symmetry Check & -0.2 & -0.3 & 0.0 & -0.02 \\
        \hline
        No Rendering Score & -0.7 & -3.5 & -3.6 & -0.03 \\
        \hline
        No Shape Network & -0.3 & -6.0 & -9.2 & +1.0 \\
        \hline
    \end{tabular}
\end{center}
\end{table*}

==> includes/nocsbenchmark.tex <==
\begin{table*}
\begin{center}
\caption{Benchmarking results on NOCS REAL \cite{wang2019normalized}. Baseline results are from sources \cite{irshad2022shapo, akizuki2021asm}. S.D. stands for shape-annotated data required for training and P.D. stands for pose-annotated data required for training. S.C. stands for the shape classification network. The results are roughly in the order of overall performance. The best result in each metric is in bold.}
\label{tab: nocspose}
    \begin{tabular}{|l| c c | c c c c c c c|}
        \hline
        Method & P.D. & S.D. & IoU25 & IoU50 & IoU75 & 5\degree 5cm & 5\degree 10cm & 10\degree 5cm & 10\degree 10cm \\
        \hline
        \hline
        NOCS \cite{wang2019normalized} & \checkmark & \checkmark & \bf{84.8} & 78.0 & 30.1 & 10.0 & 9.8 & 25.2 & 25.8 \\
        \hline
        Synthesis \cite{chen2020category} & \hfill & \hfill & -- & -- & -- & 0.9 & 1.4 & 2.4 & 5.5 \\
        \hline
        Metric Scale \cite{lee2021category} & \checkmark & \checkmark & 81.6 & 68.1 & -- & 5.3 & 5.5 & 24.7 & 26.5 \\
        \hline
        ASM-Net w/o ICP \cite{akizuki2021asm} & \checkmark & \checkmark & -- & 64.4 & 31.7 & 12.4 & -- & 37.7 & -- \\
        \hline
        \bf{\algName (Ours) w/o S.C.} & \hfill & \hfill & 82.6 & 58.3 & 37.0 & 32.4 & 33.2 & 42.2 & 43.4 \\
        \hline
        ASM-Net w/ ICP \cite{akizuki2021asm} & \checkmark & \checkmark & -- & 68.3 & 37.4 & 25.6 & -- & 43.7 & -- \\
        \hline
        \bf{\algName (Ours) w/ S.C.} & \hfill & \checkmark & 82.1 & 58.0 & 42.2 & \bf{36.5} & \bf{37.1} & 50.6 & 51.4 \\
        \hline
        ShapePrior \cite{tian2020shape} & \checkmark & \checkmark & 81.2 & 77.3 & \bf{53.2} & 21.4 & 21.4 & 54.1 & 54.1 \\
        \hline
        CenterSnap \cite{irshad2022centersnap} & \checkmark & \checkmark & 83.5 & \bf{80.2} & -- & 27.2 & 29.2 & \bf{58.8} & \bf{64.4} \\
        \hline
    \end{tabular}
\end{center}
\end{table*}

\begin{table*}
\begin{center}
\caption{Shape estimation results on NOCS REAL \cite{wang2019normalized} evaluated with Chamfer distance ($10^{-3}$). Baseline results are from sources \cite{irshad2022shapo, akizuki2021asm}. S.D. stands for shape-annotated data required for training and P.D. stands for pose-annotated data required for training. S.C. stands for the shape classification network. The results are roughly in the order of overall performance.}
\label{tab: nocsshape}
    \begin{tabular}{|l| c c | c c c c c c c|}
        \hline
        Method & P.D. & S.D. & Bottle & Bowl & Camera & Can & Laptop & Mug & Mean \\
        \hline
        \hline
        Categorical Prior \cite{tian2020shape} & \hfill & \hfill & 5.0 & 1.2 & 9.9 & 2.4 & 7.1 & 0.97 & 4.4 \\
        \hline
        \bf{\algName (Ours) w/o S.C.} & \hfill & \hfill & 2.5 & 0.86 & 9.0 & 3.7 & 3.6 & 2.8 & 3.8 \\
        \hline
        ShapePrior \cite{tian2020shape} & \checkmark & \checkmark & 3.4 & 1.2 & 8.9 & 1.5 & 2.9 & 1.0 & 3.2 \\
        \hline
        \bf{\algName (Ours) w/ S.C.} & \hfill & \checkmark & 2.8 & 0.58 & 6.8 & 1.1 & 1.2 & 3.0 & 2.6 \\      
        \hline
        CenterSnap \cite{irshad2022centersnap} & \checkmark & \checkmark & 1.3 & 1.0 & 4.3 & 0.9 & 0.7 & 0.6 & 1.5 \\
        \hline
        ASM-Net \cite{akizuki2021asm} & \checkmark & \checkmark & 0.23 & 0.06 & 0.61 & 0.15 & 0.60 & 0.10 & 0.29 \\
        \hline
    \end{tabular}
\end{center}
\end{table*}

==> includes/nocsfigures.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_1_0162_color.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_1_0162_good.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_1_0162_render_02_proc.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_1_0162_render_00_proc.png}
    \end{subfigure}
    \par\smallskip
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_2_0002_color.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_2_0002_good.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_2_0002_render_02_proc.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_2_0002_render_00_proc.png}
    \end{subfigure}
    \par\smallskip
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_3_0167_color.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_3_0167_good.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_3_0167_render_02_proc.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_3_0167_render_00_proc.png}
    \end{subfigure}
    \par\smallskip
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_4_0244_color.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_4_0244_good.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_4_0244_render_02_proc.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_4_0244_render_00_proc.png}
    \end{subfigure}
    \par\smallskip
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_5_0165_color.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_5_0165_good.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_5_0165_render_02_proc.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_5_0165_render_00_proc.png}
    \end{subfigure}
    \par\smallskip
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_6_0198_color.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_6_0198_good.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_6_0198_render_02_proc.png}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=1.0\columnwidth]{includes/figures_updated/scene_6_0198_render_00_proc.png}
    \end{subfigure}
\caption{Visualization of example NOCS REAL \cite{wang2019normalized} frames. From left to right are the color image, the color image overlaid by the depth projection of the estimated objects, back-projected measured depth image, and estimated objects from a novel viewpoint.} 
\label{fig: nocsviz}
\end{figure*}

% \begin{figure*}[ht]
%     \centering
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_1_0107_color.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_1_0107_good.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_1_0107_render_0_02_proc.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_1_0107_render_0_00_proc.png}
%     \end{subfigure}
%     \par\smallskip
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_2_0449_color.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_2_0449_good.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_2_0449_render_0_02_proc.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_2_0449_render_0_00_proc.png}
%     \end{subfigure}
%     \par\smallskip
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_5_0165_color.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_5_0165_good.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_5_0165_render_0_01_proc.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_5_0165_render_0_00_proc.png}
%     \end{subfigure}
%     \par\smallskip
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_6_0198_color.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_6_0198_good.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_6_0198_render_0_01_proc.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_6_0198_render_0_00_proc.png}
%     \end{subfigure}
% \caption{Visualization of example NOCS REAL \cite{wang2019normalized} frames. From left to right are the color image, the color image overlaid by the depth projection of the estimated objects, back-projected depth image, and estimated objects from a novel viewpoint.} 
% \label{fig: nocsviz}
% \end{figure*}

% \begin{figure*}[ht]
%     \centering
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_1_0107_color.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_1_0107_render_0_02_proc.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_1_0107_good.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_1_0107_render_0_00_proc.png}
%     \end{subfigure}
%     \par\smallskip
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_2_0449_color.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_2_0449_render_0_02_proc.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_2_0449_good.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_2_0449_render_0_00_proc.png}
%     \end{subfigure}
%     \par\smallskip
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_5_0165_color.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_5_0165_render_0_01_proc.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_5_0165_good.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_5_0165_render_0_00_proc.png}
%     \end{subfigure}
%     \par\smallskip
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_6_0198_color.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_6_0198_render_0_02_proc.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/scene_6_0198_good.png}
%     \end{subfigure}
%     \begin{subfigure}{0.24\linewidth}
%         \includegraphics[width=1.0\columnwidth]{includes/figures/processed/scene_6_0198_render_0_00_proc.png}
%     \end{subfigure}
% \caption{} 
% \label{fig: nocsviz}
% \end{figure*}
